Unleashing In-network Computing on Scientific Workloads

Many recent efforts have shown that in-network computing can benefit various datacenter applications. In this paper, we explore a relatively less-explored domain which we argue can benefit from in-network computing: scientific workloads in high-performance computing. By analyzing canonical examples of HPC applications, we observe unique opportunities and challenges for exploiting in-network computing to accelerate scientific workloads. In particular, we find that the dynamic and demanding nature of scientific workloads is the major obstacle to the adoption of in-network approaches which are mostly open-loop and lack runtime feedback. In this paper, we present NSinC (Network-accelerated ScIeNtific Computing), an architecture for fully unleashing the potential benefits of in-network computing for scientific workloads by providing closed-loop runtime feedback to in-network acceleration services. We outline key challenges in realizing this vision and a preliminary design to enable acceleration for scientific applications.

==> challenges.tex <==
\section{Challenges}
\label{sec:challenges}
%\vspace{-5pt}

%\dk{If we plan to describe challenges in accelerating (1) applications and (2) infrastructure, I think we should give backgrounds on the infrastructure in section 2.}

Modern scientific applications are highly parallel, with up to hundreds of thousands of processes generating massive amounts of data \cite{byna2012}. In simulations, particles can be modeled as key-value pairs, with the key representing a given particle attribute (e.g., energy, temperature). %As a result, duplicate keys may appear as the simulation progresses. \vyas{jun 11: not sure why duplicate keys is a high order bit for challenge?}
There are important characteristics of scientific simulations that make it challenging to use approaches from the literature to perform operations such as load balancing, caching, or indexing data. Here, we describe three: entropy, high data dimensionality, and tightly-coupled computing.

%\vyas{jun 11: one story here might be lets look 1-2 canonical solutions of in network accel has been used in datacenters. and see whether they can provide the benefits promised in 2.  right now we are talking abt abstract features without a concrete strawman/baseline to kill?} 


\mypara{C1: High entropy} 
The distribution of keys in scientific simulations can change rapidly over time. In practice, this means that choosing any static partitioning of the key space is going to result in load imbalances (i.e., runtime slowdown) during the simulation. In Figure \ref{fig:nasi-distrib}, we show the probability densities for particle energy throughout a VPIC simulation. The rapid changes shown make it challenging to find a data layout that is efficient during both data generation and data querying time (e.g., for VPIC). It also increases the difficulty of finding caching algorithms that will maintain a high hit rate (e.g., for ParSplice). This makes it hard to directly adopt adopt existing approaches for in-network caching for load balancing~\cite{sosp17-netcache, distcache-fast19} which do not assume such rapid changes in key distribution.  
%\vyas{jun 11: can we tie this to a concrete proposal from the existing datacneter literature?} 
%\dk{why existing in-net load balancing scheme (netcache) does not work?}


\mypara{C2: High-dimensional data} \TODO{Brad add relevant data?} Scientists attempt to record detailed observations of the characteristics of physical phenomena, so that detailed analyses can be performed even for aspects of a simulation that were not the initial target. As a result, scientific data is typically characterized by a large number of dimensions. For example, each VPIC particle data point consists of at least the following attributes: temperature, energy, velocity, location coordinates, magnetic field. As a result, it becomes challenging to index data so that queries to any of those attributes are answered fast.
One may think of deploying existing in-network telemetry approaches~\cite{univmon,www-nitro} based on sketches to record approximate values of the attributes. While it may work for getting individual attribute value, the current designs cannot provide telemetry data consisting of a set of attributes. This is mainly because they focus on uni-dimensional metrics of interest (e.g., entropy of source IP address distribution but not combinations of subpopulations) and a switch or data-plane centric view and ignores the network-wide visibility and aggregation.

\mypara{C3: Tightly-coupled computing} 
% seems
Many HPC applications consist of tightly coupled parallel processes that iterate together and require collective communication to make forward progress. The failure of one node to participate in this communication usually leads to a failure of the entire computation, and delayed responses can cause significant slowdown in the overall runtime of the application. As a result, the network requirements for tightly coupled applications are demanding and low latency operations are a top priority. If additional in-network components breaks the synchronous nature, it can negatively impact the overall performance. Thus, in-network compute primitives should be designed and used judiciously, and latency hiding through the careful pipelining of work may be a more appropriate alternative. 
%Thus, asynchronous communication primitives should be used judiciously, and latency hiding through the careful pipelining of work may be a more appropriate alternative. However, existing 

% \mypara{C3: Distributed data structures} 
% \TODO{change this para to synchronous operations} Discrete data structures like deques, sets, hash tables, and trees are essential in many scientific applications. These data structures fit naturally into shared-memory single-node architectures which limits scale. While distributing data structures across the memory of many nodes provides scaling,  data consistency and program semantics often limit the sequence and number of remote accesses in flight at any time. Scientific codes which frequently access distributed data structures to perform lookups or updates often have inefficient network messaging. Latencies caused by small message exchanges decrease computational efficiency and increase time to solution.
% \dk{this sounds like a generic problem in dist sys.}

% \vyas{jun 11: why is this diff from any other ML workload??} 

% \vyas{jun 11: meta point i like these are concrete, but perhaps we need to take a concrete strawman to poke at for each or in sumamry?}


==> related.tex <==
\section{Background and Related Work}
\label{sec:background}
\vspace{-5pt}

This project naturally draws from a number of related computer science disciplines and is influenced heavily by requirements of modern HPC architectures; these topics are discussed below.

\subsection{Programmable Network Capabilities}
\label{sec:bg-prog-net}
%\vspace{-5pt}

Recent advances in programmable switch ASICs~\cite{www-tofino, www-xpliant} and programmable NICs~\cite{www-innova2,www-liquidio, Mellanox17}  become key enablers that allow the data plane to perform computation directly on the packet beyond its traditional role, i.e., packet forwarding. Many studies have shown that various network functions such as load balancing~\cite{sigcomm17-silkroad}, network monitoring~\cite{www-barefoot_int, sigcomm17-marple}, and distributed applications such as sequencers~\cite{osdi16-nopaxos} and key-value 
stores~\cite{sosp17-netcache, nsdi18-netchain,asplos17-incbricks}
can be implemented on programmable switches to improve application performance and network efficiency.
Remote Direct Memory Access (RDMA) is another key capability supported by commodity programmable NICs~\cite{Mellanox17, www-innova2}.
The ability of RDMA to lower CPU consumption has been leveraged by prior work to create applications such as key-value
stores~\cite{atc13-pilaf,sigcomm14-herd, nsdi14-farm}, distributed shared-memory~\cite{nsdi14-farm}, transactional systems~\cite{eurosys16-drtm, sosp15-farm}, and distributed NVM systems~\cite{atc17-octopus,socc17-dspm}. 
Recent work by Sandia National Laboratories, called INCA~\cite{sc19-inca}, has proposed a new deadline-free, bump-in-the-wire SmartNIC architecture and has shown that such a NIC architecture can accelerate scientific applications and kernels.

Prior work from our team has demonstrated that we can leverage programmable network capabilities to improve the performance and effectiveness of various applications: (1) enhancing network monitoring tasks by realizing universal sketching on programmable switches~\cite{sigcomm16-univmon}, (2) enabling a distributed caching layer on programmable switches for key-value stores~\cite{distcache-fast19}, and (3) accelerating replicated transactional storage systems~\cite{sigcomm18-hyperloop}.
In recent work, we have proposed an external memory architecture for programmable switches that demonstrates a novel use of RDMA, which allows a programmable switch to leverage external DRAM on connected servers to address the memory constraints of in-network compute resources and support memory-intensive services~\cite{hotnets18-gem, sigcomm20-tea}.

\subsection{Accelerating Scientific Workflows}
%\vspace{-5pt}
Prior work by the team has focused on understanding scientific workloads, and redesigning systems infrastructure to achieve significant speedups during the data processing and data analysis phases, without requiring changes to the logic of the scientific applications. The following subsections describe two prior projects in this space: application-aware caching and in-situ data indexing.

\subsubsection{Application-aware Caching Policies}
%\vspace{-5pt}
ParSplice uses a hierarchy of in-memory caches and a single persistent key-value store to store the atomic coordinates corresponding to local energy minima encountered by a large number of independent dynamical trajectories. This memoization workload is pervasive across scientific applications that (1) require re-using large numbers of calculations from prior timesteps or expensive offline analysis (e.g. equation of state lookup tables) or (2) leverage physics-based rules to rapidly reduce a large multi-dimensional search space stored in lookup tables into a smaller number of candidate values (e.g. HipMer). The fine-grained data annotation capabilities provided by key-value storage is a natural match for these types of scientific simulations. In prior work we demonstrated that Mantle, an application-specific policy engine, can implement physics-based cache eviction and replacement strategies that reduced the cache memory footprint by 32-66\% while providing nearly identical trajectory simulation runtimes using ParSplice~\cite{8411024}. Unfortunately, large-scale simulations saturate the capacity and bandwidth capabilities of a single node cache and we need more effective data management techniques as we scale the cache across larger node counts. 
Extending this work to improve distributed cache lookup performance and cache injection performance are critical to further improving the scalability of ParSplice on real systems. 

\subsubsection{In-situ data indexing}
\label{sec:deltafs}
%\vspace{-5pt}
%\begin{wrapfigure}{r}{0.41\textwidth}
%\centering
%\includegraphics[width=0.39\textwidth]{figures/tr-query.pdf}
%\vspace{-10pt}
%\caption{VPIC runs on LANL's Trinity cluster show $1740\times$ query speedup with DeltaFS.}
%The baseline reader uses all CPU cores to search particles in parallel, but DeltaFS queries use a single core.}
%\label{fig:exp-tr-query}
%\vspace{-10pt}
%\end{wrapfigure}

Scientific data is often persisted in an order that is not ideal for subsequent analysis.
To allow applications to operate on an arbitrarily large number of files without the need for data sorting, we developed the DeltaFS distributed file system \cite{Zheng18, Zheng17}.
DeltaFS allows each application to individually control the amount of computing resources dedicated to the service.
Our experiments show that DeltaFS can process two orders of magnitude more operations than Lustre and GPFS \cite{Zheng15}.
A popular scientific application that can benefit from DeltaFS is VPIC (\S\ref{sec:vpic}). VPIC
outputs particle data for each simulated time step out of order. Scientists, however, are mostly interested in accessing all data for a given particle, e.g., to study its trajectory. To speed up such queries DeltaFS indexes data in-situ as it is written to storage. Our experiments show at least $1,740\times$ speedup when particle data is accessed through DeltaFS (Figure \ref{fig:exp-tr-query}). The proposed work aims to leverage the experience our team built on data indexing, in combination with in-network acceleration, to generalize this approach, decreasing time to discovery for more DOE applications and miniapps~\cite{pennant}.
%\vspace{-5pt}

\subsection{Sketch-based Telemetry}
%\vspace{-5pt}

Sketches are useful for many telemetry tasks such as detection of heavy hitter  flows with significant impact on total traffic~\cite{CMSketch,SpaceSavings,CountSketch,HashPipe,sigcomm16-univmon} or capacity~\cite{k-ary,revsketch,sigcomm16-univmon}, cardinality estimation of the number of distinct traffic flows~\cite{F0sketch,sigcomm16-univmon}, entropy estimation for different header distributions \cite{Lall:2006}, and anomaly  detection for identifying destinations that receive an unexpected surge in traffic~\cite{OpenSketch}.
Our recent work  UnivMon~\cite{sigcomm16-univmon} and NitroSketch~\cite{liu2019nitrosketch} provide extensions to support a range of these tasks, rather than a specialized sketch per task.
At a high-level, sketches are  approximate data structures to estimate various statistics of a given streaming workload, which   are   designed to  achieve guaranteed fidelity for the estimated statistics with low memory footprint.   They typically consists of    arrays of counters, and use a set of independent hash functions to update these counters. To illustrate this  structure of sketches,  consider the Count-Min Sketch (CMS)~\cite{CMSketch}. CMS maintains $d$ arrays of $w$ counters each. On its \emph{Update} procedure, it computes $d$ independent hash values from the packet's flow identifier (e.g., 5-tuple). Each such hash provides an offset within one of the $d$ arrays, and CMS then increases the corresponding 
counters. This data structure can then be used for a number of estimation tasks. Specifically, the estimate for a given flow's size is the minimum value among the corresponding counters for this flow. Using these per-flow estimates, we can compute other derived statistics such as quantiles.   

\subsection{Hardware Accelerators for HPC Storage Systems Software}
\label{sec:bg-off-hpc-storage}
%\vspace{-5pt}

Complex storage software stacks providing erasure coding, end-to-end checksums, compression, and data indexing are unable to expose all of the underlying device performance due to insufficient compute resources on storage servers. Although processors with large core counts are widely available, single task performance and memory bandwidth per task have grown much more slowly than core counts. Common storage system operations that require multiple passes over memory (e.g., many compression and indexing algorithms) are already unable to keep pace with fast storage devices and networks. 
Similarly, popular software stacks that enable the composition of multiple compute-intensive and memory-intensive operations, such as checksum, compression, and erasure coding capabilities \cite{zfs, leveldb},
are unable to fully leverage the storage bandwidth provided by the tens of NVME drives available in current solid-state disk enclosures.
%
%\begin{wrapfigure}{r}{0.5\textwidth}
%\includegraphics[width=0.49\textwidth]{figures/fast-endpoint-write-for-incsams.eps}
%\vspace{-5pt}
%\caption{I/O performance of the popular ZFS file system using 3 different processing platforms. ZFS is configured to calculate checksums and erasure coding (RAIDZ2 algorithm).
%Performance results are ordered by system memory bandwidth where Intel Platinum provides the highest performance, and AMD Naples provides the lowest.
%Performance results are ordered by system memory bandwidth with the dual socket Intel Platinum server (12 memory channels of bandwidth) providing the highest performance, the AMD Rome system (8 channels) providing less performance, and the AMD Naples system (8 channels total, 2 channels local to each core) providing the least performance.
%Even with high-end processors the software stack is unable to expose device levels of performance shown as Raw NVME write.}
%\label{storage:a}
%\vspace{-10pt}
%\end{wrapfigure}
%
Figure~\ref{storage:a} shows how storage system performance decreases as critical data protection tasks are added to the software stack. To alleviate storage system software bottlenecks, architectures that place additional compute resources along the storage data path become increasingly attractive.

Computational storage, in the process of standardization~\cite{snia-cs-draft}, is a promising avenue to alleviate processing bottlenecks within storage system software via on-device computation.
On-device computation allows data processing to occur nearest to the data, and began with exploring the ability of devices to carry out arbitrary computation~\cite{928624,5348819}. Two decades later, prototype devices are emerging with limited computational power targeted to specialized tasks, such as object stores~\cite{seagate_kinetic}, key-value stores~\cite{samsung_kvssd}, in-line data compression~\cite{6131148} and compaction~\cite{8843040}.
In our own work we have used FPGAs as computational storage processors to accelerate high-quality compression~\cite{lanl-eideticom-csp}.  
We have published a branch of the ZFS file system that supports compression tasks offloaded onto a standards-compliant NVME computational storage devices~\cite{www-zfs-noload}, and continue to work with the nCorium storage platform that places FPGAs on DIMMs to accelerate erasure coding~\cite{ncorium19}.

